Combinatorial-hybrid Optimization for Multi-agent Systems under Collaborative Tasks

Multi-agent systems can be extremely efficient when working concurrently and collaboratively, e.g., for transportation, maintenance, search and rescue. Coordination of such teams often involves two aspects: (i) selecting appropriate sub-teams for different tasks; (ii) designing collaborative control strategies to execute these tasks. The former aspect can be combinatorial w.r.t. the team size, while the latter requires optimization over joint state-spaces under geometric and dynamic constraints. Existing work often tackles one aspect by assuming the other is given, while ignoring their close dependency. This work formulates such problems as combinatorial-hybrid optimizations (CHO), where both the discrete modes of collaboration and the continuous control parameters are optimized simultaneously and iteratively. The proposed framework consists of two interleaved layers: the dynamic formation of task coalitions and the hybrid optimization of collaborative behaviors. Overall feasibility and costs of different coalitions performing various tasks are approximated at different granularities to improve the computational efficiency. At last, a Nash-stable strategy for both task assignment and execution is derived with provable guarantee on the feasibility and quality. Two non-trivial applications of collaborative transportation and dynamic capture are studied against several baselines.

==> contents/cases_copy.tex <==
\section{Two Concrete Use Cases}\label{sec:cases}
To clarify the problem formulation described in Sec.~\ref{sec:problem},
two use cases of multi-agent systems
that can be modeled by the CHO framework are presented first in this section,
of which the detail setup and results are given in Sec.~\ref{sec:experiments}.


%==============================
\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{figures/transportation_mode.pdf}
  \caption{Illustration of three different modes associated with the use case of object transportation
    described in Sec.~\ref{subsec:dynamic-capture}:
    Long-Side Pushing (\textbf{Left}), Short-Side Pushing (\textbf{Middle}),
    and Pushing Diagonally (\textbf{Right}).
    Robots (green circles) form different coalitions and modes
    for the transportation of boxes (blue rectangles).
    \textcolor{blue}{
    In each mode, robots choose different parameters 
    to form a hybrid plan for transporting objects.
    }
  }
  \label{fig:transportation_mode}
  \vspace{-2mm}
  \label{fig:transportation_mode}
\end{figure}
%==============================
%==============
\subsection{Collaborative Transportation}\label{subsec:col-transport}
Consider the problem in which a team of~$N$ agents is tasked to move~$M$
identical rectangular boxes
from their initial positions to target positions in a cluttered workspace,
as illustrated in Fig.~\ref{}. \todo{Add figure}
The state of a box is determined by its center~$(x_m, y_m)$ and the its orientation~$\psi_m$,
of which the target position is given by~$(x_m^\star,y_m^\star)$.

The agents can make contact at specific points on the box and push the box forward
by applying bounded pushing force $F_n\in[0,\, F_{\max}]$.
Note that the set of all possible contact points is given
and different combinations of contact points result in different system dynamics
and thus different modes~$\Xi=\{\xi_k\}$. \todo{How many modes?}
As shown in Fig.~\ref{}, the box can be pushed by different number of agents in different modes,
where the parameters are the applied forces~$\rho_k=\{F_n\}$.
Clearly, more agents lead to a higher degree of controllability. 
Moreover, under certain scenarios with narrow passages,
a sequence of different modes with distinct parameters might be required
to move a box to its target position.


%==============================
\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{figures/capture_mode.pdf}
  \caption{Illustration of three different modes associated with the use case of dynamic capture
    described in Sec.~\ref{subsec:dynamic-capture}:
    Pure Pursuit (\textbf{Left}), Hide and Attack (\textbf{Middle}),
    and Enclosure (\textbf{Right}).
    Pursuers (blue triangles) form different coalitions and modes
    for the capture of evaders (red circles).
    \textcolor{blue}{
    In each mode, pursuers choose different parameters (cyan diamond) 
    to form a hybrid plan for capturing the evaders.
    }
  }
  \label{fig:capture_mode}
  \vspace{-2mm}
  \label{fig:capture_mode}
\end{figure}
%==============================

%==============
\subsection{Dynamic Capture}\label{subsec:dynamic-capture}
Consider the problem of ``N vs. M'' dynamic capture,
which involves~$N$ pursuers and~$M$ evaders in a cluttered 2D workspace.
Their states and velocities are denoted by~$(x_n(t), v_n(t))$ and $(y_m(t), v_m(t))$, respectively.
The pursuers and evaders have the \emph{same} maximum velocity~$v_{\max}$,
meaning that collaborations are required for the pursuers to catch the evaders.
Namely, there is a capture task associated with each evader,
of which the set of goal states is where the distance between the evader and any pursuer
is less than a given distance.
The evader simply moves in the opposite direction of all pursers, weighted their relative distances.

In addition, as shown in Fig.~\ref{fig:capture_mode},
there are three parameterized modes~$\Xi=\{\xi_1,\,\xi_2,\, \xi_3\}$ for each task:
(i) \emph{Pure Pursuit}.
In this mode, the pursuers follow the ``line-of-sight'' strategy to move directly towards the assigned evader,
i.e., $v_n=v_{\max}\, \texttt{point}(\{x_n\},\,\rho_1)$,
where~$\texttt{point}(\cdot)$ is the unit vector from~$x_n$ to the
parameter~$\rho_1\in \mathbb{R}^2$ as determined by the position of assigned evaders,
while avoiding collision with other pursers and obstacles.
(ii) \emph{Hide and Attack}.
In this mode,
the pursuers conceal themselves behind obstacles until the assigned evader appears,
and then capture the evader by encircling with other pursuers,
i.e., $v_n = \texttt{nav}(\{x_n\},\, \rho_2)$,
where~$\texttt{nav}(\cdot)$ is a given navigation function that guides
the pursuer to a hiding or attacking position~$\rho_2\in \mathbb{R}^2$
given the position of other pursuers in the workspace.
(iii) \emph{Enclosure}:
In this mode,
the pursers drive the assigned evader into a corner by reducing the region of advantage for the evader,
until the evader is captured.
i.e., $v_n = \texttt{corner}(\{x_n\},\,\rho_3)$,
where~$\texttt{corner}(\cdot)$ is an optimization algorithm that generates the optimal velocity
that maximizes the region of advantage given the position of all pursuers~$\{x_n\}$ and~$\rho_3\in \mathbb{R}^2$.
Consequently, each pursuer should choose its hybrid plan as the sequence of mode,
coalition and the associated parameter,
such that all evaders can be caught as fast as possible.


==> contents/structure.tex <==
\subsection{Hierarchical Structure}\label{subsec:structure}
\todo{To discuss}
Instead of a flat tree structure, a hierarchical structure is proposed to
separate the core modules.
More specifically, it consists of four main parts:
\begin{enumerate}
\item[(i)] coalition formation (Nash-K stable?);
\item[(ii)] behavior planning (discrete search?);
\item[(iii)] geometric optimization (Nonliner program NLP?);
\item[(iv)] motion control (distributed-MPC?).
\end{enumerate}

\todo{key challenges to be addressed}
\begin{enumerate}
\item In step (i), utility functions needed for coalition formation are generally unknown before solving subsequent steps.
\item In step (ii), how to create discrete abstractions under each mode automatically, to facilitate search?
\item In step (iii), solving NLP is normally the most expensive step.
  How to design feasibility check or compute relaxed bounds in step (ii), to limit the number of NLPs solved?
\item Is step (iv) necessary? Is it possible to propose a general method for distributed motion planning,
  e.g., to ensure collision avoidance.
\item ...\todo{maybe Zili knows the best}
\end{enumerate}

\todo{Of course, we are proposing an efficient framework, instead of proving everything.}

